Do You See What I See? A Qualitative Study Eliciting High-Level Visualization Comprehension

Designers often create visualizations to achieve specific high-level analytical or communication goals. These goals require people to naturally extract complex, contextualized, and interconnected patterns in data. While limited prior work has studied general high-level interpretation, prevailing perceptual studies of visualization effectiveness primarily focus on isolated, predefined, low-level tasks, such as estimating statistical quantities. This study more holistically explores visualization interpretation to examine the alignment between designers' communicative goals and what their audience sees in a visualization, which we refer to as their comprehension. We found that statistics people effectively estimate from visualizations in classical graphical perception studies may differ from the patterns people intuitively comprehend in a visualization. We conducted a qualitative study on three types of visualizations -- line graphs, bar graphs, and scatterplots -- to investigate the high-level patterns people naturally draw from a visualization. Participants described a series of graphs using natural language and think-aloud protocols. We found that comprehension varies with a range of factors, including graph complexity and data distribution. Specifically, 1) a visualization's stated objective often does not align with people's comprehension, 2) results from traditional experiments may not predict the knowledge people build with a graph, and 3) chart type alone is insufficient to predict the information people extract from a graph. Our study confirms the importance of defining visualization effectiveness from multiple perspectives to assess and inform visualization practices.

==> sec-statistics.tex <==

\begin{figure}[htbp]
\centering
\includegraphics[width=0.75\columnwidth]{figs/bars.png}
\vspace{-5pt}
\caption{Summary of participants' responses on statistical quantities and patterns in their comprehension.}
\vspace{-10pt}
\label{fig:statistic}
\end{figure}

% 
% 
One of our additional matching criteria in participant's comprehension is to observe their responses with salient identified patterns and statistics. Based on low-level task coding from participants' responses, we explored \textit{what type of patterns people saw in the three graph types and those vary among the graph's design dimension?}
% 
We observed the participants conveyed eight different types of patterns and statistics---\emph{anomalies, compute derived values, cluster, correlate, distribution, extremum, range, and trend} in their responses.
As shown in \autoref{fig:statistic}, we quantified the statistics and patterns from participant responses across three visualization types.


We centralize our discussion here on \autoref{fig:statistic} and investigate whether statistics and pertain to a specific \textbf{graph type}. We observed \textit{trend} has the maximum count (123) in the line graph, correlation (103) in the scatterplot, and extremum (120) in the bar graph. This pattern of reporting suggests that participants mostly search for a particular pattern in a given type of graph. For example, discrete value and extremum in bar graphs, the trend in line graphs, and correlation in scatterplots. Additionally, distribution and cluster to the scatterplot, computation of derived value to both line and bar graph. Based on the participants' response when they missed achieving the designer's goal, extremum, computing the derived value on `change over time' and the trend is used across all three graph types. Surprisingly, participants searched for correlations in both line and bar graphs.

We further explored how patterns identified by participants varied with the \textbf{data and graph composition type}. We observed a high variation of identified pattern type for single-class graphs, as shown in \autoref{fig:statistic}. Multi-class graphs mention comparatively more `compare' with less varied pattern types. We did not observe any specific details in the bar graphs. However, multi-class line graph responses are more trend-focused, such as change, increase-decrease or upward-downward trend, spike, increase, peak-valley, and multi-class scatterplot responses are more varied with cluster, correlate, trend, and extremum. Furthermore, people did not comprehend the use of juxtaposed graphs, and we noted \textit{compare} a lot fewer composite graphs. \textit{Compare} term was equally used among all graph dimensions except single-class graphs. Multi-class juxtaposed kine graphs response include trends and adjectives such as upward-downward, non-monotonic, oscillation, ubiquitous, steep decrease, stable, and similar. As expected, however, in lesser occurrences, \textit{Compare} combined with other statistics, such as correlation, trend, and extremum.

There are cases where participants missed and failed to identify the salient patterns. People did not discuss extremum, computed derived value, or characterizing distribution in the scatterplot. To our wonder, we observed many responses where participants failed to mention correlation for salient patterns in scatterplots. In multi-class line graphs, people miss the trend in clustering patterns, distribution, clusters, and correlation. People's responses showed no mention of the distribution and order of bar values.


\begin{quote}
    ``\textit{What is the relationship between the age of the car with odometer readings? What model of car has the lowest and highest odometer readings? What price of the car has the lowest/highest odometer reading?}'' [Nursing Student, 21], on \autoref{fig:stimulus_mc} (b)
\end{quote}



